Compress, Then Prompt: Improving Accuracy-Efficiency Trade-off of LLM Inference with Transferable Prompt

While the numerous parameters in Large Language Models (LLMs) contribute to their superior performance, this massive scale makes them inefficient and memory-hungry. Thus, they are hard to deploy on commodity hardware, such as one single GPU. Given the memory and power constraints of such devices, model compression methods are widely employed to reduce both the model size and inference latency, which essentially trades off model quality in return for improved efficiency. Thus, optimizing this accuracy-efficiency trade-off is crucial for the LLM deployment on commodity hardware. In this paper, we introduce a new perspective to optimize this trade-off by prompting compressed models. Specifically, we first observe that for certain questions, the generation quality of a compressed LLM can be significantly improved by adding carefully designed hard prompts, though this isn't the case for all questions. Based on this observation, we propose a soft prompt learning method where we expose the compressed model to the prompt learning process, aiming to enhance the performance of prompts. Our experimental analysis suggests our soft prompt strategy greatly improves the performance of the 8x compressed LLaMA-7B model (with a joint 4-bit quantization and 50% weight pruning compression), allowing them to match their uncompressed counterparts on popular benchmarks. Also, we demonstrate that these learned prompts can be transferred across various datasets, tasks, and compression levels. Hence with this transferability, we can stitch the soft prompt to a newly compressed model to improve the test-time accuracy in an ``in-situ'' way.

==> intro.tex <==
\section{Introduction}\label{sec:intro}
The emergence of Large Language Models (LLMs)~\cite{radford2018improving, radford2019language, brown2020language, zhang2022opt, llama}, boasting billions of parameters, has revolutionized the field of Natural Language Processing (NLP).
Remarkably, LLMs can be directly deployed for new tasks without additional training.
In this paradigm, termed in-context
learning~\cite{xieexplanation,min2022rethinking}, LLMs are controlled through user-provided natural language specifications of the task, or \emph{prompts}, which illustrate how to complete a task. 
Equipped with the in-context learning ability, we only need to serve a single large model to efficiently handle a wide array of tasks.
However, LLMs come with substantial inference costs~\cite{chen2023frugalgpt,wu2023fast}, making them challenging to serve. 
As LLM becomes larger and larger, running LLM inference on the cloud may require multiple graphics processing units (GPUs), which is prohibitively expensive for many users. 
Consequently, it is crucial to provide LLM inference service on accessible hardware, such as a single GPU, which possesses limited computational capacity and memory.
This mismatch between the LLM's resource-intensive nature and the capabilities of commonly available hardware leads to considerable latency, posing challenges in terms of cost, memory, and processing time.

To make LLMs executable on the extremely economic case of a single GPU, it is critical to reducing both the computation and memory usage during inference. This challenge has spurred research into LLM compression techniques. For instance, one sparsifies LLM parameters so that each input sample only triggers a fraction of tensor operations and thereby enhances model throughput~\cite{frantar2023sparsegpt,liu2023DejaVu}.
Furthermore, we can quantize LLM parameters into fewer bits~\cite{nagel2020up,dettmers2022llm,xiao2022smoothquant,frantar2022gptq}, resulting in a more efficient use of computation and memory. 
These compression methods reduce the computational and memory complexity at the cost of giving less accurate outputs. 
Thus, there is often an inevitable trade-off between accuracy and efficiency, resulting in a noticeable reduction in the model's accuracy and, consequently, the overall performance benefits of LLMs.
As shown in Figure \ref{fig: motivation_example}, 
the full model (LLaMA-7B) is able to provide accurate answers to all three simple questions.
However,
the pruned model generates answers that are unrelated and off-topic to these simple questions.


Previous LLM compression works usually fix the input text while compressing the model weight in a manner that minimizes the effects of compression.
On a separate note, the prompt is essentially a task description attached to the original input text, which affects LLMs outputs.
Intuitively, we can also utilize the prompt to help the compressed model to generate more relevant answers.
However, to the best of our knowledge, this perspective is not explored for LLMs. 
In view of such, we ask: \emph{for a compressed model, can we design a prompt that informs the model of its compressed state and helps it correct its predictions accordingly?}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{figures/motivation_examples.pdf}
    \caption{A compression-aware prompt enables compressed LLMs to regain the commonsense. Here the human designed hard prompt is ``\textbf{Please carefully examine the weight matrix within the model, as it may contain errors. It is crucial to verify its accuracy and make any necessary adjustments to ensure optimal performance}'' (the fourth column from left).
    We highlight the improved answers with the green color.
    }
    \label{fig: motivation_example}
\end{figure}

We posit that the way inputs are fed to these models can profoundly influence their output quality. 
As shown in Figure \ref{fig: motivation_example},
we manually attach the prompt ``\emph{Please carefully examine the weight matrix within the model, as it may contain errors. It is crucial to verify its accuracy and make any necessary adjustments to ensure optimal performance}'' to the original question.
The prompted pruned model, i.e., ``LLaMA-7B (62.5\% sparsity) w./ Hard Prompt'' in Figure \ref{fig: motivation_example}, shows a significant improvement in its responses, although not all of them are accurate or complete.
Our investigation suggests that compressed LLMs can understand the instruction and magically adjust to generate more relevant responses for some of the questions.
Furthermore, this manually-crafted prompt only conveys that the model weight might be inaccurate, without considering the dataset, compression methods, or tasks. This finding highlights the considerable potential for the transferability of this ``compression-aware prompt'' across datasets, compression levels, and tasks.
Despite the potential, this manually designed prompt is not consistently effective.
Inspired by previous learnable prompt works \cite{li2021prefix, lester2021power},
we hypothesize that by involving the compressed weight in the prompt learning process, a learnable prompt could potentially surpass the performance of the manually-designed prompt, while maintaining the transferability. 
Building upon this insight, we introduce a paradigm of prompt learning that seeks to train additive prompt tokens on a compressed LLM to enhance its accuracy. 
We underscore that the primary distinction between our prompt learning approach and previous prompt tuning frameworks \cite{li2021prefix, lester2021power} is that earlier methods mainly utilized the prompt to adapt the model for specific downstream tasks. In contrast, the learned prompt in this paper resembles the hard prompt in Figure \ref{fig: motivation_example}, as it allows compressed LLMs to regain commonsense and can be transferred between various datasets, compression methods, and tasks.

Our empirical analysis reveals that this strategic utilization of prompts can elevate the performance of compressed LLMs to the level of, and occasionally even beyond, their original models. In a promising development, we also observe a certain degree of transferability of these learned prompts across different datasets, tasks, and compression levels. These findings not only illuminate new possibilities for improving the trade-off between efficiency and accuracy in LLM inference but also underscore the potential role of input editing in enhancing the performance of compressed models. 
